BAXTER: Bi-modal Aerial-Terrestrial Hybrid Vehicle for Long-endurance Versatile Mobility: Preprint Version

Unmanned aerial vehicles are rapidly evolving within the field of robotics. However, their performance is often limited by payload capacity, operational time, and robustness to impact and collision. These limitations of aerial vehicles become more acute for missions in challenging environments such as subterranean structures which may require extended autonomous operation in confined spaces. While software solutions for aerial robots are developing rapidly, improvements to hardware are critical to applying advanced planners and algorithms in large and dangerous environments where the short range and high susceptibility to collisions of most modern aerial robots make applications in realistic subterranean missions infeasible. To provide such hardware capabilities, one needs to design and implement a hardware solution that takes into the account the Size, Weight, and Power (SWaP) constraints. This work focuses on providing a robust and versatile hybrid platform that improves payload capacity, operation time, endurance, and versatility. The Bi-modal Aerial and Terrestrial hybrid vehicle (BAXTER) is a solution that provides two modes of operation, aerial and terrestrial. BAXTER employs two novel hardware mechanisms: the M-Suspension and the Decoupled Transmission which together provide resilience during landing and crashes and efficient terrestrial operation. Extensive flight tests were conducted to characterize the vehicle's capabilities, including robustness and endurance. Additionally, we propose Agile Mode Transfer (AMT), a transition from aerial to terrestrial operation that seeks to minimize impulses during impact to the ground which is a quick and simple transition process that exploits BAXTER's resilience to impact.

==> BAXTER_Full_Paper/fig/BAXTER_Components_Table.tex <==

\begin{table} 
    \centering
    \caption{System Components of BAXTER}
    \scalebox{0.9}{
        \begin{tabular}{c||c c}
            \textbf{System}&\textbf{Type}&\textbf{Hardware}\\
            \hline
            \textbf{Aerial Mobility}
            &Actuator&8x T-Motor F60 2500KV\\
            &ESC& 8x Hobbywing XRotor 40A\\
            &Propeller& 8x 7"x4.5"\\
            &Flight Controller&Pixhawk PX4\\
            \hline
            \textbf{Terrestrial Mobility}
            &Actuator&2xJGB37-520\\
            &Controller&2x Pololu JRK 18v19\\
            &Wheel&228mm diameter\\
            \hline\hline
            Onboard Computer & & NVIDIA Jetson TX2\\
            \hline
            Sensors &Odometry&QSF Pro\\
            &1D Lidar(Altitude)&TeraRanger Evo Mini\\
            \hline
            Battery&&4S 6000mAh\\
            \hline
        \end{tabular} \label{fig:components}
    }
\end{table}


==> BAXTER_Full_Paper/fig/BAXTER_Iteration.tex <==
\begin{table} 
    \centering
    \caption{Summary of Hybrid Platform Iterations from KAIST USRG
    \todo{This and other figures may look better formatted with the subfigure environment}}
    \scalebox{1}{
        \begin{tabularx}{1\textwidth} { 
              | >{\centering\arraybackslash}X 
              | >{\centering\arraybackslash}X 
              | >{\centering\arraybackslash}X | }
        \hline
            1. Model 1 "TUMBLER"&2. Model 2 "HEXWING"&3. Model 4 "BAXTER"\\
            \hline
            \includegraphics[width = 0.13 \textwidth]{BAXTER_Full_Paper/fig/M1_Render.jpg}
            \includegraphics[width = 0.13 \textwidth]{BAXTER_Full_Paper/fig/M1_Pic.png}
            &\includegraphics[width = 0.13 \textwidth]{BAXTER_Full_Paper/fig/M2_Render.png}
            \includegraphics[width = 0.13 \textwidth]{BAXTER_Full_Paper/fig/M2_Pic.jpg}
            &\includegraphics[width = 0.13 \textwidth]{BAXTER_Full_Paper/fig/M4_Render.png}
            \includegraphics[width = 0.13 \textwidth]{BAXTER_Full_Paper/fig/M4_Pic.jpg}\\
            \hline
            \begin{tabular}{@{}>{\textbullet{}}p{0.3\textwidth}}
               A proof of concept for a spherical protective cage\\
               A proof of concept for separately-powered Terrestrial mode\\
               A simple, manual-controlled hybrid aerial vehicle with minimal capabilities for terrestrial mobility
            \end{tabular}
            &
            \begin{tabular}{@{}>{\textbullet{}}p{0.3\textwidth}}
               A proof of concept for a spherical unit sub-assemblies including power units for both modes.\\
               A scale up from previous version to incorporate light on-board sensors\\
               Introduction of terrestrial mode operation
            \end{tabular}
            &
            \begin{tabular}{@{}>{\textbullet{}}p{0.3\textwidth}}
               A proof of concept of the M-Suspension and Decoupled Transmission for endurance to impact and agile mode transition\\
               A scale up from precious version to incorporate heavier on-board sensors and processor units
            \end{tabular} \\
            \hline
        \end{tabularx} \label{table:iteration}
    }
\end{table}

==> BAXTER_Full_Paper/fig/BAXTER_landing_physics.tex <==
\begin{table}[h] 
\vspace{-.800cm}
    \centering
    \caption{Simplified Kinematics Model for BAXTER's Agile Mode Transition {\color{red} Ali: Sahand or Chris or Inhwan/Taeyon: Please create this table outside the latex, and make the figures and notations inside the figures larger and readable. this  is an imporntat table.} 
    %\chris{need to unify the model type: physics model? dynamic model? kinematic model? simple kinematic model? (currently noted as [!physics!])}
    }
    \scalebox{0.83}{
        \begin{tabular}{|c|c|c|c|}
        \hline
        1. Free Fall&2. Initial Impact&3. Roll&4. Final Impact\\
        \hline
        \includegraphics[width = 0.25 \textwidth]{fig/phy_1.png}&\includegraphics[width = 0.25 \textwidth]{fig/phy_2.png}&\includegraphics[width = 0.25 \textwidth]{fig/phy_3.png}&\includegraphics[width = 0.25 \textwidth]{fig/phy_4.png}\\
        \hline 
        $\begin{aligned}
         v_{1x} =& v_{0x} \\
         v_{1y} =& -\sqrt{2g\Delta h}
        \end{aligned}$
        &
        $\begin{aligned}
         &\Vec{d_2} \times \Vec{v_1} = \Vec{d_2} \times \Vec{v_2} + I\Vec{\omega_2} \\
         &-\Vec{v_2} + \Vec{\omega_2}\times\Vec{d} + \Vec{\omega} \times \Vec{r}= \Vec{0}
        \end{aligned}$
        &
        $\begin{aligned}
         \frac{1}{2}mv_2^2+\frac{1}{2}Iw_2^2+mgh_2&\\= \frac{1}{2}mv_3^2+\frac{1}{2}Iw_3^2&\\
         -\Vec{v_3} + \Vec{\omega_3}\times\Vec{d} + \Vec{\omega} \times \Vec{r} = \Vec{0}&
        \end{aligned}$
        &
        $\begin{aligned}
         \Vec{d_4} \times \Vec{v_3} + I\Vec{\omega_3} =&\\
         \Vec{d_4} \times \Vec{v_4} +& I\Vec{\omega_4}\\
         -\Vec{v_4} + \Vec{\omega}\times\Vec{r} + \Vec{\omega_4}\times&\Vec{d} = \Vec{0}
        \end{aligned}$
        \\
        \hline
        \end{tabular} \label{table:physics}
    }
    \vspace{-.600cm}
\end{table}
